Do Neural Networks for Segmentation Understand Insideness?

The insideness problem is an aspect of image segmentation that consists of determining which pixels are inside and outside a region. Deep Neural Networks (DNNs) excel in segmentation benchmarks, but it is unclear if they have the ability to solve the insideness problem as it requires evaluating long-range spatial dependencies. In this paper, the insideness problem is analysed in isolation, without texture or semantic cues, such that other aspects of segmentation do not interfere in the analysis. We demonstrate that DNNs for segmentation with few units have sufficient complexity to solve insideness for any curve. Yet, such DNNs have severe problems with learning general solutions. Only recurrent networks trained with small images learn solutions that generalize well to almost any curve. Recurrent networks can decompose the evaluation of long-range dependencies into a sequence of local operations, and learning with small images alleviates the common difficulties of training recurrent networks with a large number of unrolling steps.

==> broader_impact.tex <==

\vspace{\baselineskip}
\noindent {\bf Statement of Broader Impact. }
This work provides insights about why DNNs do not generalize well to segmenting families of curves that were not included in the training set, and investigates the representations that lead to general solutions and how to learn them. We contribute to establishing the reductionist approach to understanding DNNs, where specific problem components are investigated by minimizing the interference of other factors. The reductionist approach allows to open the “black box” of DNNs and analyze precisely how DNNs represent specific aspects of visual understanding. 



Furthermore, we add to the body of work on DNN's failure modes by demonstrating a potential vulnerability with the insideness problem.
This creates a risk of pointing out vulnerabilities that can be exploited with negative societal consequences~\cite{heaven2019deep}; for instance, in the case of visual tasks, demonstrating ways to fool surveillance or self-driving cars \cite{comiter2019attacking}. However, understanding specific vulnerabilities is crucial towards building more robust, explainable networks. 


%It is of critical importance to make progress on understanding the internal functioning and decision-making process of DNNs. This will facilitate applications in which human lives are dependent upon the outcomes of the DNNs. Examples are DNNs for self-driving cars, disease diagnostics from medical images, and surveillance. A common criticism of the viability of DNNs in these applications is in fact the lack of explainability~\cite{davenport2019potential}.


% *cite: https://www.ncbi.nlm.nih.gov/pmc/articles/PMC6616181/

%**cite:https://www.nature.com/articles/d41586-019-03013-5

%***cite: https://www.belfercenter.org/publication/AttackingAI.

%This research can also lead to improvements of state-of-the-art methods in applications that require understanding of complex spatial relationships. Insideness can be helpful when there are few cues available besides the boundaries of the objects, ie. when there is lack of texture and color, such as in cartoons or sketches, or when objects have different textures and shapes from those seen during training. Furthermore, while object recognition requires analysis of local image regions, insideness requires DNNs to capture long-range spatial relationships that are crucial for robust image understanding. Thus, our work demonstrates how DNNs can be trained to capture a general solution to a more ‘abstract’ semantic segmentation problem. 
%Potential negative impacts (ideas for what to write about -- should be rigorous)
 

==> dilation_vis.tex <==
\renewcommand{\arraystretch}{0}

\begin{figure}[t]
  \footnotesize
  \begin{tabular}{c}
     {\bf Examples of Feature Maps  of the Dilated Conv. DNN }\\
     \includegraphics[width=0.47\textwidth]{./fig/dilation_vis/15.pdf}
  \end{tabular}
\caption{\emph{Visualization of the Feature Maps of the Learnt 2-layer Convolutional LSTM.} [Feature maps of the second are inverted]}
\end{figure}


==> fig/abstract.tex <==

A key component of visual cognition is the understanding of spatial relationships among objects. Albeit effortless to our visual system, state-of-the-art artificial neural networks struggle to distinguish basic spatial relationships among elements in an image. As shown here, deep neural networks (DNNs) trained with hundreds of thousands of labeled examples cannot accurately distinguish whether pixels lie inside or outside 2D shapes, a problem that seems much simpler than image segmentation. In this paper, we sought to analyze the capability of ANN to solve  such  inside/outside problem using an analytical approach. We  demonstrate that it is a mathematically tractable problem and that two previously proposed algorithms, namely the Ray-Intersection Method and the Coloring Method, achieve perfect accuracy when implemented in the form of DNNs. 

%In the next step, we trained ANNs with labeled 2D shapes categorized by complexity and found that the discriminability of inside/outside relationships is inversely proportional to the complexity of the input shape. We can then infer that ANNs do not solve image segmentation using insideness as a sub-component, since they do not understand this last problem.

% ----- VERSION 1 -----
%A key component of visual cognition is the understanding of spatial relationships among objects. Albeit effortless to our visual system, state-of-the-art artificial neural networks struggle to distinguish basic spatial relationships among elements in an image. As shown here, deep neural networks (DNNs) trained with hundreds of thousands of labeled examples cannot accurately distinguish whether pixels lie inside or outside 2D shapes. In this paper, we sought to analyze the learnability of such  inside/outside problem using an analytical and an experimental approach. We first demonstrated that it is a mathematically tractable problem and that two previously proposed algorithms, namely the Ray-Intersection Method and the Coloring Method, achieve perfect accuracy when implemented in the form of deep neural networks. In the next step, we trained DNNs with labeled 2D shapes categorized by complexity and found that the discriminability of inside/outside relationships is inversely proportional to the complexity of the input shape. [Which are the implications of our findings?]

% ----- VERSION 2 -----
% A key component of visual cognition is the understanding of spatial relationships among objects. Albeit effortless to our visual system, state-of-the-art deep neural networks struggle to distinguish basic spatial relationships of objects. As we demonstrate here, deep neural networks trained with hundreds of thousands of labeled examples cannot accurately distinguish whether pixels lie inside or outside 2D shapes. Nonetheless, we can show that this is a mathematically tractable problem and that two previously proposed algorithms, namely the Ray-Intersection Method and the Coloring Method, achieve perfect accuracy when implemented in the form of deep neural networks. The reasons why artificial networks can't learn how to solve the inside/outside problem remain unknown but our results suggest that the discriminability of such spatial relationship is inversely proportional to the complexity of the input. [Which are the implications of our findings?]


% ----- VERSION 3 -----
% A key component of visual cognition is the understanding of spatial relationships among objects. Albeit effortless to our visual system, state-of-the-art deep neural networks struggle to distinguish basic spatial relationships of objects, such as whether an object is inside or outside another object. To shed light in this problem, here we investigated it using an analytic and an experimental perspective. First, we demonstrated that the inside/outside problem is mathematically tractable. In the next step, we showed that two previously proposed algorithms, namely the Ray-Intersection Method and the Coloring Method, can be implemented in the form of deep neural networks, being able to solve the inside/outside problem with perfect accuracy. Finally, after training our neural networks with a dataset containing hundreds of thousands of 2D shapes separated by degree of complexity, we found that the discriminability of inside/outside relationships is inversely proportional to the complexity of the input. [Which are the implications of our findings?]

% ----- VERSION 4 -----
% A key component of visual cognition is the understanding of spatial relationships among objects. Albeit effortless to our visual system, state-of-the-art deep neural networks perform very poorly when trained to distinguish basic spatial relationships among elements in an image. To discern whether an object is inside or outside another object, the inside/outside problem, has been a big challenge for machine learning algorithms. Here we revisited this problem using an analytical and an experimental approach. First we demonstrate that the inside/outside problem is mathematically tractable nice problem. Then we show that two previously proposed algorithms, namely the Ray-Intersection Method and the Coloring Method, can be implemented in the form of deep neural networks. Further, we show that the two neural networks are able to solve the inside/outside problem with perfect accuracy. Finally, based on experimental results, we conjecture that discriminability of inside/outside relationships is inversely proportional to the complexity of the input shape. [Which are the implications of our findings?]

%Image segmentation aims at grouping pixels that belong to the same object or image region. Deep Neural Networks (DNNs) excel in current segmentation benchmarks by adding  including  are  segmentation with object recognition . However, benchmarks for image segmentation include a mix of task 


==> fig/lstm_output_shaping.tex <==
\renewcommand{\arraystretch}{0}

\begin{figure}[t!]
  \centering
  \begin{tabular}{c}
    \scriptsize
        \ \ \quad {\bf Input} 
       \  \ \quad {\bf t=0}
      \ \ \ \ \quad {\bf t=5}
       \ \ \ \quad {\bf t=10}
       \ \ \quad {\bf t=15}
       \ \ \ \quad {\bf t=20}
       \ \ \ \quad {\bf t=25} 
       \ \ \ \quad {\bf t=30}
       \ \ \ \quad {\bf t=35}
       \ \ \ \quad {\bf t=40}
       \ \ \ \quad {\bf t=45}
       \ \ \quad {\bf t=50}
       \ \ \ \quad {\bf t=55}\\
     \includegraphics[width=0.99\textwidth]{./fig/lstm_small_output_vis/act_2.pdf} \\
         \includegraphics[width=0.99\textwidth]{./fig/lstm_small_output_vis/act_8.pdf} \\
         \includegraphics[width=0.99\textwidth]{./fig/lstm_small_output_vis/act_12.pdf} \\
  \includegraphics[width=0.99\textwidth]{./fig/lstm_small_output_vis/act_5.pdf} \\
        \includegraphics[width=0.99\textwidth]{./fig/lstm_small_output_vis/act_10.pdf} \\

  \end{tabular}
\caption{\emph{Output of the \emph{2-LSTM}, Trained on Small Images ($18\times 18$ pixels).} Each row corresponds to the output of the network for different images and each column to a different time step. The first column corresponds to the input image. Note that the network implements the coloring routine because it expands the ``outside'' region and blocks the expansion at the border of the curve.  }
\label{output_visSuppLSTM_shaping_paper}
\end{figure}


==> fig/lstm_shaping.tex <==
\renewcommand{\arraystretch}{0}

\begin{figure}[t!]
  \centering
  \begin{tabular}{c}
    \scriptsize
     \ \ \ \ \ \ \quad {\bf t=0} 
     \ \ \ \ \ \quad {\bf t=5}
      \ \ \ \ \quad {\bf t=10}
      \ \ \ \quad {\bf t=15}
      \ \ \ \ \quad {\bf t=20}
      \ \ \ \ \quad {\bf t=25} 
      \ \ \ \ \quad {\bf t=30}
      \ \ \ \ \quad {\bf t=35}
      \ \ \ \ \quad {\bf t=40}
      \ \ \ \ \quad {\bf t=45}
      \ \ \ \quad {\bf t=50}
      \ \ \ \ \quad {\bf t=55}\\
     \includegraphics[width=0.99\textwidth]{./appendix_folder/fig/lstm_shaping_vis/activation_fig_0.pdf} \\
  \end{tabular}
\caption{\emph{Activation Maps of the Learnt Representations by \emph{2-LSTM}, Trained on Small Images ($18\times 18$ pixels).} Each row corresponds to a different layer and each column to a different time step. Note that the network implements the coloring routine because it expands the ``outside'' region and blocks the expansion at the border of the curve. Interestingly, the implementation of the coloring routine is different from the one theoretically derived in the paper, which is depicted in Fig.~\ref{figMAthLSTM} in Appendix~\ref{Additional_Figures_and_Visualizations}. Observe that for the solution displayed in this figure, the cell state has the same trend as the hidden state but in the derived solution the cell state is equal to $\neg \boldsymbol{X}$.  This demonstrates that there are different ways of implementing the coloring routine. Also, the feature maps of the hidden state of the \emph{RNN} (not displayed here) are very similar to the ones displayed in this figure for the second LSTM.   }
\label{visSuppLSTM_shaping_paper}
\end{figure}


==> lstm_math_vis.tex <==
\renewcommand{\arraystretch}{0}

\begin{figure}[t]
  \begin{tabular}{c}
    \footnotesize
     {\bf \hspace{0.2cm} t=0 \hspace{0.75cm} t=4 \hspace{0.8cm}t=8 \hspace{0.8cm}t=12\hspace{0.6cm} t=16\hspace{0.65cm} t=20} \\
     \includegraphics[width=0.47\textwidth]{./fig/lstm_vis/math15.pdf}
  \end{tabular}
\caption{\emph{Visualization of Convolutional LSTM with the Ideal Parameters.}}
\end{figure}


==> lstm_vis.tex <==
\renewcommand{\arraystretch}{0}

\begin{figure}[t]
  \begin{tabular}{c}
    \footnotesize
     {\bf \hspace{0.2cm} t=0 \hspace{0.75cm} t=4 \hspace{0.8cm}t=8 \hspace{0.8cm}t=12\hspace{0.6cm} t=16\hspace{0.65cm} t=20} \\
     \includegraphics[width=0.47\textwidth]{./fig/lstm_vis/15.pdf}
  \end{tabular}
\caption{\emph{Activation Maps of the Learnt Representations by \emph{2-LSTM}.} Each row depicts a different layer and each column a time step. Fig.~\ref{visSuppLSTM} shows more examples.}
\label{visLSTM}
\end{figure}


==> qualitative.tex <==
\renewcommand{\arraystretch}{0}

\begin{figure}[t]
  \begin{tabular}{c}
    \footnotesize
     {\bf  \hspace{-0.05cm}   Dilated  \hspace{0.55cm} Feed-Forward  \hspace{0.6cm} UNet  \hspace{0.95cm} 2-LSTM} \\
    %\includegraphics[width=0.47\textwidth]{./fig/qualitative/15.pdf}\\ [-0.15cm]
    %\includegraphics[width=0.47\textwidth]{./fig/qualitative/16.pdf}\\ [-0.15cm]
            \includegraphics[width=0.47\textwidth]{./fig/qualitative/35.pdf}
  \end{tabular}
\caption{\emph{Qualitative Examples from the Digs dataset.} Networks trained in $24$-Polar and Spiral dataset fail to segment in the Digs dataset. Fig.~\ref{exSuppQuak} shows more examples.}
 \label{exQuak}
\end{figure}


==> quantitative1.tex <==
\renewcommand{\arraystretch}{0}

\begin{figure*}[t]
  \footnotesize
  \begin{tabular}{c@{\hspace{-0.01cm}}c@{\hspace{-0.01cm}}c@{\hspace{-0.01cm}}c}
        \includegraphics[width=0.24\textwidth]{./fig/quantitative//1.pdf}&
        \includegraphics[width=0.24\textwidth]{./fig/quantitative//2.pdf}&
        \includegraphics[width=0.24\textwidth]{./fig/quantitative//Dilated.pdf}&
        \includegraphics[width=0.24\textwidth]{./fig/quantitative//2-LSTM.pdf}\\
        (a) & (b) & (c) & (d) 
  \end{tabular}
\caption{\emph{Results in the Polar Dataset.} Intra-dataset evaluation using (a) per pixel accuracy and (b) per image accuracy. Evaluation using the testing set of each Polar datasets for (c)~\emph{Dilated} and (d)~\emph{2-LSTM} networks.}
\label{resQuant1paper}
\end{figure*}

